Computer-Assisted Design of Accelerated Composite Optimization Methods: OptISTA

The accelerated composite optimization method FISTA (Beck, Teboulle 2009) is suboptimal by a constant factor, and we present a new method OptISTA that improves FISTA by a constant factor of 2. The performance estimation problem (PEP) has recently been introduced as a new computer-assisted paradigm for designing optimal first-order methods. In this work, we present a double-function stepsize-optimization PEP methodology that poses the optimization over fixed-step first-order methods for composite optimization as a finite-dimensional nonconvex QCQP, which can be practically solved through spatial branch-and-bound algorithms, and use it to design the exact optimal method OptISTA for the composite optimization setup. We then establish the exact optimality of OptISTA under the large-scale assumption with a lower-bound construction that extends the semi-interpolated zero-chain construction (Drori, Taylor 2022) to the double-function setup of composite optimization. By establishing exact optimality, our work concludes the search for the fastest first-order methods, with respect to the performance measure of worst-case function value suboptimality, for the proximal, projected-gradient, and proximal-gradient setups involving a smooth convex function and a closed proper convex function.

==> shuvos_preamble.tex <==
%% In case fonts are not rendered properly, please do the following:
%% 1. In Document > Settings..., under Language > Encoding, choose "Other" 
%% and select "Language Default (no inputenc)".
%% 2. Simply uncheck "Use LaTeX font encoding" and no fontenc line will be added.

% Make sections heading bold sans serif
%\usepackage{graphicx,psfrag,amsfonts,verbatim,  mathtools}
\usepackage{graphicx,psfrag,amsfonts,verbatim,fullpage,mathtools}
\usepackage[hidelinks]{hyperref}

\usepackage{xurl}

% \usepackage[linesnumbered,ruled,vlined]{algorithm2e}

%\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
%\SetCommentSty{mycommfont}

\usepackage{bbm}

\usepackage{dsfont}

\usepackage[framemethod=default]{mdframed}



\global\mdfdefinestyle{vert_line_shuvo}
{
linecolor=black, 
linewidth=2pt, 
%innerleftmargin=5pt,
%leftmargin=13pt,
%innertopmargin=0pt,
%innerbottommargin=0pt,
%innerrightmargin=0pt,
%skipabove=0pt, 
%skipbelow=0pt, 
topline=false, 
nobreak=true,
bottomline=false, 
rightline=false
} 

\global\mdfdefinestyle{algorithm_box_shuvo}
{
linecolor=black, 
linewidth=1pt, 
innerleftmargin=1pt,
%leftmargin=13pt,
innertopmargin=5pt,
innerbottommargin=5pt,
innerrightmargin=1pt,
%skipabove=0pt, 
%skipbelow=0pt, 
%topline=false, 
nobreak=true,
%bottomline=false, 
%rightline=false
} 



\usepackage{ upgreek } % for regularized fonts

\usepackage[bbgreekl]{mathbbol}
\DeclareSymbolFontAlphabet{\mathbbm}{bbold}
\DeclareSymbolFontAlphabet{\mathbb}{AMSb}%
\usepackage[bb=px]{mathalfa}
\usepackage{bm}
\usepackage{mathtools}

\PassOptionsToPackage{obeyFinal}{todonotes}
% \usepackage{bm} % for bold math
\usepackage{todonotes}

\usepackage{abstract} % Make abstract

\theoremstyle{plain}
\newtheorem{thm}{\protect\theoremname}
\theoremstyle{plain}
\newtheorem{cor}{\protect\corollaryname}
\theoremstyle{plain}
\newtheorem{lem}{\protect\lemmaname}
\theoremstyle{plain}
\newtheorem{assumption}{Assumption}
\theoremstyle{plain}
\newtheorem{remark}{Remark}
\theoremstyle{definition}
\newtheorem{defn}{\protect\definitionname}
\theoremstyle{plain}
\newtheorem{prop}{\protect\propositionname}
\theoremstyle{remark}
\newtheorem{rem}{\protect\remarkname}
\theoremstyle{plain}
\newtheorem{conjecture}{Conjecture}


\usepackage{babel}
%\providecommand{\definitionname}{Definition}
\providecommand{\lemmaname}{Lemma}
\providecommand{\propositionname}{Proposition}
\providecommand{\theoremname}{Theorem}
\providecommand{\corollaryname}{Corollary}
%\providecommand{\remarkname}{Remark}



% using parskip for nice paragraph spacing 
\usepackage{parskip}
% these are to fix the paragraph spacing for theorems, only used if parskip package is used
\begingroup
\makeatletter
   \@for\theoremstyle:=definition,remark,plain\do{%
     \expandafter\g@addto@macro\csname th@\theoremstyle\endcsname{%
        \addtolength\thm@preskip\parskip
     }%
   }
\endgroup
\usepackage{parskip}

\usepackage{diagbox}

\definecolor{commentcolor}{RGB}{74,112,35}

% Make section titles bold
\renewcommand\abstractnamefont{\bfseries\sffamily}
% section title fonts
\usepackage{titlesec}
\def\sectionfont{\sffamily\Large\bfseries\boldmath}
\def\subsectionfont{\sffamily\large\bfseries\boldmath}
\def\paragraphfont{\sffamily\normalsize\bfseries\boldmath}
\titleformat*{\section}{\sectionfont}
\titleformat*{\subsection}{\subsectionfont}
\titleformat*{\subsubsection}{\paragraphfont}
\titleformat*{\paragraph}{\paragraphfont}
\titleformat*{\subparagraph}{\paragraphfont}
\usepackage[small,labelfont={bf,sf}]{caption}  % Change captions
\setlength{\abovecaptionskip}{0em}



\usepackage{multirow}
\setlength{\captionmargin}{20pt}
\usepackage{enumitem}
\setlist{nolistsep}

% Tables
\usepackage{booktabs}           % Nicer Tables
\usepackage{adjustbox} % To adjust table length


\usepackage{titling}
\pretitle{\begin{center}\LARGE \bfseries\sffamily}
\posttitle{\par\end{center}\vskip 2em}
\preauthor{\begin{center}
\large \lineskip 2em%
\begin{tabular}[t]{c}}
\postauthor{\end{tabular}\par\end{center}}
\predate{\begin{center}\large}
\postdate{\par\end{center}}

\usepackage{tikz}
\usetikzlibrary{fit, arrows, shapes, positioning, shadows, matrix, calc}
\usepackage[]{subfig}

\usepackage{amssymb}

% pgfplot
\RequirePackage{luatex85}
%\documentclass[tikz]{standalone}
% Default preamble
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{polar}
\usepgfplotslibrary{smithchart}
\usepgfplotslibrary{statistics}
\usepgfplotslibrary{dateplot}
\interfootnotelinepenalty=10000



\allowdisplaybreaks




